DYNAMITE: Dynamic Defense Selection for Enhancing Machine Learning-based Intrusion Detection Against Adversarial Attacks

The rapid proliferation of the Internet of Things (IoT) has introduced substantial security vulnerabilities, highlighting the need for robust Intrusion Detection Systems (IDS). Machine learning-based intrusion detection systems (ML-IDS) have significantly improved threat detection capabilities; however, they remain highly susceptible to adversarial attacks. While numerous defense mechanisms have been proposed to enhance ML-IDS resilience, a systematic approach for selecting the most effective defense against a specific adversarial attack remains absent. To address this challenge, we propose Dynamite, a dynamic defense selection framework that enhances ML-IDS by intelligently identifying and deploying the most suitable defense using a machine learning-driven selection mechanism. Our results demonstrate that Dynamite achieves a 96.2% reduction in computational time compared to the Oracle, significantly decreasing computational overhead while preserving strong prediction performance. Dynamite also demonstrates an average F1-score improvement of 76.7% over random defense and 65.8% over the best static state-of-the-art defense.

==> background.tex <==
\section{Background}\label{sec:background}

\subsection{Adversarial Attacks}
%Adversarial attacks are techniques used to manipulate machine learning models by adding small, intentional perturbations to input data. These perturbations are often imperceptible to humans but can cause models to produce incorrect or undesirable outputs. The following are common adversarial attack methods:
Adversarial attacks manipulate ML models by adding small, intentional perturbations to input data. Overall, we select six widely used white-box and black-box adversarial attacks:

\textbf{Fast Gradient Sign Method (FGSM)} \cite{goodfellow2014explaining}: FGSM is a white-box attack that generates adversarial examples by applying a single perturbation in the direction of the gradient of the loss function with respect to the input. 
%It is computationally efficient and effective for generating adversarial attacks. The simplicity of FGSM makes it one of the most widely used methods for testing the robustness of machine learning models.

\textbf{Basic Iterative Method (BIM)} \cite{kurakin2018adversarial}: BIM is a white-box attack and an iterative extension of FGSM. It applies multiple small perturbations, recalculating gradients after each step, to accumulate stronger adversarial effects on the input. 
%By taking smaller steps iteratively, BIM generates more precise and effective adversarial examples compared to FGSM.

\textbf{DeepFool (DF)} \cite{moosavi2016deepfool}: DF is a white-box attack and an iterative method that aims to find the smallest perturbation required to misclassify an input. It linearizes the decision boundaries of the model to calculate efficient perturbations. 
%DeepFool is particularly effective in crafting minimally perturbed adversarial examples, making it useful for evaluating a model’s vulnerability.

\textbf{Projected Gradient Descent (PGD)} \cite{madry2017towards}: PGD is a white-box attack that extends FGSM by iteratively applying perturbations while projecting the perturbed input back to a constrained range to ensure the perturbations remain bounded. 
%PGD is considered one of the strongest first-order adversarial attacks and is often used as a benchmark for evaluating model robustness.

\textbf{Auto Projected Gradient Descent (AutoPGD)} \cite{croce2020reliable}: AutoPGD is a white-box attack that automates the process of tuning the step size for PGD attacks. It uses adaptive step sizes to ensure efficient generation of strong adversarial examples. 
%AutoPGD provides a more reliable method for generating adversarial examples by addressing the limitations of manual step-size selection in PGD.

\textbf{Zeroth Order Optimization (ZOO)} \cite{chen2017zoo}: ZOO is a black-box attack that approximates gradients using finite differences, a method that estimates gradients by perturbing individual input features. Unlike other black-box attacks, ZOO utilizes a coordinate-wise optimization approach, which systematically updates one input dimension at a time, allowing it to efficiently handle high-dimensional input spaces. This makes ZOO particularly effective in scenarios where the adversary can only query the model’s output probabilities and where computational efficiency is critical, such as when attacking APIs or proprietary systems with restricted access. 
% It can generate adversarial examples without direct access to the model's gradients, making it suitable for attacking black-box systems. 
%ZOO is particularly useful in scenarios where the attacker can only query the model’s outputs, such as APIs or proprietary systems.

\subsection{Adversarial Defenses}
Defense mechanisms aim to protect ML models from adversarial attacks by enhancing their robustness or reducing the effectiveness of adversarial perturbations. We select nine different defense methods from three types of defense categories:
%into training-based, model-modification, and supplementary approaches.

\subsubsection{Adversarial Training (AT)}
Adversarial training (AT) involves generating adversarial examples during the training process and incorporating them into the training set to make the model robust against such attacks. AT is selected because it directly improves robustness by training models on adversarially perturbed data, making them resilient to similar attacks.

\textbf{Projected Gradient Descent AT} \cite{madry2017towards}: PGD-generated adversarial examples are used in the training process to fine-tune the model. This approach is widely recognized as the most effective and commonly used "regular" adversarial training method, providing a strong baseline for defending against adversarial attacks by iteratively generating and countering perturbations during training.
% This method significantly improves resistance to white-box attacks like PGD. By directly training the model on challenging adversarial examples, this approach enhances the model's ability to generalize under attack conditions.

\textbf{Interpolated AT} \cite{lamb2019interpolated}: Interpolated AT addresses the common issue of reduced clean data performance observed in standard adversarial training by improving the model's generalization to both adversarial and clean inputs. It achieves this by interpolating between clean and adversarial examples during training, allowing the model to strike a balance between robustness and accuracy.

\textbf{TRadeoff-inspired Adversarial DEfense via Surrogate-loss Minimization (TRADES)} \cite{zhang2019theoretically}: TRADES addresses the trade-off between robustness to adversarial examples and accuracy on clean data, which is a common limitation in adversarial training. By introducing a surrogate loss function, TRADES explicitly balances these two objectives, ensuring the model maintains competitive performance on clean inputs while improving its adversarial robustness.

\textbf{Free AT} \cite{shafahi2019adversarial}: Free AT reduces the computational cost of adversarial training by reusing gradient computations within a single training step to simultaneously update model parameters and generate adversarial examples. This approach eliminates the need for additional forward and backward passes typically required in adversarial training, significantly reducing overhead. However, as the generated adversarial examples are constrained by the limited gradient updates, it lacks the robustness to defend against stronger attacks.

\textbf{Gaussian Augmenter} \cite{zantedeschi2017efficient}: Gaussian noise is added to inputs during training to simulate adversarial perturbations. This method increases robustness by exposing the model to noisy variations. By adding random noise, the Gaussian augmenter enables the model to learn to disregard minor distortions in the input data. 

\subsubsection{Modify the Training Process}
These methods adapt the training process or objective to make models inherently robust against adversarial attacks. Modification of the training process is included as it enables the optimization of loss functions or training strategies to mitigate vulnerabilities.

\textbf{Defensive Distillation (DD)} \cite{papernot2016distillation}: 
%DD reduces the sensitivity of models to small input changes. 
DD uses a two-step process where a model is trained to predict soft labels (probabilities) and then a second model is trained using these soft labels, making gradients harder to exploit. This method creates smoother decision boundaries, making adversarial perturbations less effective.

\textbf{Robust Soft Label Adversarial Distillation (RSLAD)} \cite{zi2021revisiting}: RSLAD refines Defensive Distillation by optimizing the soft labels of the teacher model to better align with adversarially perturbed inputs. This ensures the student model learns to generalize under adversarial conditions. Variants like RSLAD10 and RSLAD100 use different intensities of adversarial examples, balancing robustness and computational cost. 
% These approaches allow fine-tuning of robustness levels based on specific application requirements.

\subsubsection{Input Transformation Techniques}
These methods focus on preprocessing or transforming input data to mitigate the impact of adversarial perturbations before it is fed into the model. Input transformation techniques are selected because they provide an effective, model-agnostic way to defend against adversarial attacks by disrupting the structured patterns of adversarial noise, thereby reducing the likelihood of successful exploitation.

\textbf{Feature Squeezing} \cite{xu2017feature}: This method reduces the resolution or complexity of input data (e.g., reducing color bit depth) to limit the space available for adversarial manipulation. By simplifying inputs, feature squeezing effectively reduces the variability that attackers can exploit.

\textbf{Gaussian Noise} \cite{kassam2012signal}: Adding Gaussian noise to inputs disrupts adversarial perturbations. This preprocessing step makes it harder for adversarial examples to mislead the model. The randomness introduced by Gaussian noise creates a form of input regularization that improves model robustness.

